Fair-Share Allocations for Agents with Arbitrary Entitlements

We consider the problem of fair allocation of indivisible goods to $n$ agents, with no transfers. When agents have equal entitlements, the well established notion of the maximin share (MMS) serves as an attractive fairness criterion, where to qualify as fair, an allocation needs to give every agent at least a substantial fraction of her MMS. In this paper we consider the case of arbitrary (unequal) entitlements. We explain shortcomings in previous attempts that extend the MMS to unequal entitlements. Our conceptual contribution is the introduction of a new notion of a share, the AnyPrice share (APS), that is appropriate for settings with arbitrary entitlements. Even for the equal entitlements case, this notion is new, and satisfies $APS \ge MMS$, where the inequality is sometimes strict. We present two equivalent definitions for the APS (one as a minimization problem, the other as a maximization problem), and provide comparisons between the APS and previous notions of fairness. Our main result concerns additive valuations and arbitrary entitlements, for which we provide a polynomial-time algorithm that gives every agent at least a $\frac{3}{5}$-fraction of her APS. This algorithm can also be viewed as providing strategies in a certain natural bidding game, and these strategies secure each agent at least a $\frac{3}{5}$-fraction of her APS.

==> acks.tex <==
%\section*{Acknowledgement}
\begin{acks}

%\thanks{
The full version of this paper is available at \url{https://arxiv.org/abs/2103.04304} .

%Authors' email addresses:
%MB: moshe@microsoft.com ;
%TE: tomer.ezra@gmail.com ; 
%UF: uriel.feige@weizmann.ac.il .

Tomer Ezra’s research is supported by the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation program (grant agreement No. 866132), and by the Israel Science Foundation (grant number 317/17).
Part of the work was conducted at Microsoft Research, Herzeliya.%}
\end{acks}


==> allocationalgorithm.tex <==



%\begin{itemize}
%		\item

\mbc{need to turn this section to a discussion section. This should be part of a discussion at the end regarding  the philosophical meaning of "shares" (common units to measure outcomes) and what do we learn from the approximation results - that this algorithm has a solution that gives each agent at least something.   }

If one is to use the share notion as a deterministic solution concept (rather than ex-post guarantee), then the natural approach is to do lex-max (which is also Pareto efficient). This applies not only to APS but also to other notions of shares, such as MMS.

\uf{For agents with 0 share, the scaling below cannot be done. By convention, if get~0 value this is equivalent to getting one unit of share. Geting more value is equivalent to infinity, but we will need different notions of infinity.}\mbc{How do we take care of multiple zero shares? }

As for 3 agents maximin cannot be guaranteed (and since $APS>=MMS$), we cannot guarantee everyone his APS share  for three agents or more. (3.16).
		We thus need approximation and then do lex-max.
	
%\end{itemize}

%\mbc{this is general algorithm that works for any share}
\begin{algorithm}
	%\captionsetup{labelfont={sc,bf}, labelsep=newline}
	\caption{Lex-max share-based allocation algorithm\label{alg:lex-max}
	}
	\begin{algorithmic}
		\STATE $s_i = $ share of agent i
		\STATE scale each $v_i$ by $\frac{1}{s_i}$. (with the convention that $0/0=1$. )
		\STATE return the lex-max allocation with respect scaled valuations
	\end{algorithmic}
\end{algorithm}

\uf{Alert that this is not a polynomial time algorithm}


\te{In later sections we show existence results which imply that the allocation returned by Algorithm~\ref{alg:lex-max} guarantees at least those fractions of the shares.}





==> relations.tex <==
\section{OLD: Relations between shares for Additive }
Give a theorem summarizing many  results for additive:
$$proportional\geq truncated  \geq anyPrice \geq b-pessimistic\ share\geq maximin(b)\geq \frac{1}{2} anyPrice$$ 
Every inequality is strict for some instances. 

claim follows from:
\begin{itemize}
	\item Observation (2.2 +2.3 from old writeup) that anyprice $\geq  b$-pessimistic share (as it is so for) the $p/q$-share for any $p/q\leq b$.
	\item truncated proportional $\geq$ anyprice (3.1)
	\item 2*maximin $\geq$  anyprice (3.3) 	
\end{itemize}


